Handling Ontology Gaps in Semantic Parsing

The majority of Neural Semantic Parsing (NSP) models are developed with the assumption that there are no concepts outside the ones such models can represent with their target symbols (closed-world assumption). This assumption leads to generate hallucinated outputs rather than admitting their lack of knowledge. Hallucinations can lead to wrong or potentially offensive responses to users. Hence, a mechanism to prevent this behavior is crucial to build trusted NSP-based Question Answering agents. To that end, we propose the Hallucination Simulation Framework (HSF), a general setting for stimulating and analyzing NSP model hallucinations. The framework can be applied to any NSP task with a closed-ontology. Using the proposed framework and KQA Pro as the benchmark dataset, we assess state-of-the-art techniques for hallucination detection. We then present a novel hallucination detection strategy that exploits the computational graph of the NSP model to detect the NSP hallucinations in the presence of ontology gaps, out-of-domain utterances, and to recognize NSP errors, improving the F1-Score respectively by ~21, ~24% and ~1%. This is the first work in closed-ontology NSP that addresses the problem of recognizing ontology gaps. We release our code and checkpoints at https://github.com/amazon-science/handling-ontology-gaps-in-semantic-parsing.

==> conclusions_bak.tex <==
The current studies in Neural Semantic Parsing (NSP) revolve around improving performance on closed-world benchmarks, but they do not take into account the trustworthiness of the model in a real world scenario where the model is used to serve answers to users of QA system.
In such scenario the NSP models will likely hallucinate the understanding of the input utterances that cannot be represented in its target ontology.

Hallucinations undermine the trustworthiness of NSP models by delivering incorrect answers, especially in sectors like healthcare, finance, and legal where error costs are high.
To test NSP models under this more realistic scenario, we propose the Hallucination Simulation Framework (HSF), where we programmatically introduce ontology gaps in the test sets of existing closed-world semantic parsing datasets.
We propose the Hallucination Detection Model, a neural architecture that analyzes an NSP model at inference time to detect hallucinations using several hallucination detection signals.
We propose to use the activations as a novel hallucination detection signal, and when it is combined with other signals such as the confidence score, Monte Carlo Dropout leads the HDM to obtain an improvement of Macro F1-Score in detecting hallucinated MRLs of 21\% in out-of-ontology, 1\% in NSP Errors, and 24\% in zero-shot OOD detection.
% Thanks to HSF, different solutions to mitigate hallucinations can be explored to obtain more trustworthy NSP models.

%However, the hallucination detection is still a hard problem especially in the case of recognizing out-of-ontology utterances.


% Because every state-of-the-art NSP model are prone to generate hallucinated answers and we consider important to take this aspect into account in all NSP benchmark.

% Detecting hallucinations still an hard problem in Generative NLP, 
% The current studies in Neural Semantic Parsing revolve around improving performance on standard benchmark, but in that work we raise up that performance on benchmark which apply the CWA \ref{sec:cwa} are not sufficient to measure the quality of an NSP model.

% Because every state-of-the-art NSP model are prone to generate hallucinated answers and we consider important to take this aspect into account in all NSP benchmark.
% For that reason, we present the HSF that poses a NSP model at the center of a simulation, HSF imposes a methodology based on two datasets one to train the NSP model over a subset of the ontology and then a second dataset (HDD) to stimulate hallucinations explointing the remaining part of the ontology.
% %The HSF breaks up the CWA \ref{sec:cwa}, which assumes that the symbols present in its training set (ontology) are sufficient to represent each input sentence and that there are no other symbols outside of it.


% Having a strategy to stimulate hallucinations, let us to build a neural network able to detect them.



% Given that, we artificially remove a portion of these symbols dropping the associated sentences from the training and development sets of our NSP model, to simulate an ontology gap.
% Given the \textit{Closed World Assumption} described in the Section \ref{sec:cwa}, considering a sentence which requires at least one symbol of the missing ontology, the model will always produce an MRL, since it is unable to refuse the MRL production and it will attempt to find the best match with underlying ontology which results in hallucinating relations.



